Surface Parametrization of Nonsimply Connected Planar B\'ezier Regions

A technique is described for constructing three-dimensional vector graphics representations of planar regions bounded by cubic B\'ezier curves, such as smooth glyphs. It relies on a novel algorithm for compactly partitioning planar B\'ezier regions into nondegenerate Coons patches. New optimizations are also described for B\'ezier inside-outside tests and the computation of global bounds of directionally monotonic functions over a B\'ezier surface (such as its bounding box or optimal field-of-view angle). These algorithms underlie the three-dimensional illustration and typography features of the TeX-aware vector graphics language Asymptote.

==> cad-10+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix cad-10+0_0.pdf}%
}%


==> cad-10.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 95.347250pt{}%
\kern 131.482250pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{12.000000}{14.400000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-65.741125,47.673625)(-0.500000,-0.500000){\includemovie[3Dlights=Headlamp,text={\includegraphics[hiresbb]{"\ASYprefix cad-10+0_0".pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -179.803304906384198603,3Droll=0,3Droo=179.803304906384198603,3Dbg=1 1 1,3Djscript=\ASYprefix cad-10+0.js]{128.48pt}{92.345pt}{\ASYprefix cad-10+0.prc}}


==> cad-11+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix cad-11+0_0.pdf}%
}%


==> cad-11.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 95.347250pt{}%
\kern 130.478510pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{12.000000}{14.400000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-65.239255,47.673625)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{"\ASYprefix cad-11+0_0".pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -178.724477161057365038,3Droll=0,3Droo=178.724477161057365038,3Dbg=1 1 1,3Djscript=\ASYprefix cad-11+0.js]{127.47625pt}{92.345pt}{\ASYprefix cad-11+0.prc}}


==> cad-12+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix cad-12+0_0.pdf}%
}%


==> cad-12.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 95.347250pt{}%
\kern 130.478510pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{12.000000}{14.400000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-65.239255,47.673625)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{"\ASYprefix cad-12+0_0".pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -178.724477161057365038,3Droll=0,3Droo=178.724477161057365038,3Dbg=1 1 1,3Djscript=\ASYprefix cad-12+0.js]{127.47625pt}{92.345pt}{\ASYprefix cad-12+0.prc}}


==> cad-14+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix cad-14+0_0.pdf}%
}%


==> cad-14.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 273.010990pt{}%
\kern 391.453500pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{12.000000}{14.400000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-195.726750,136.505495)(-0.500000,-0.500000){\includemovie[3Dlights=Headlamp,text={\includegraphics[hiresbb]{"\ASYprefix cad-14+0_0".pdf}},label=,toolbar=false,3Daac=13.460232192607241686,3Dc2c=0 0 1,3Dcoo=0 0 -967.766031575216516103,3Droll=0,3Droo=967.766031575216516103,3Dbg=1 1 1,3Djscript=\ASYprefix cad-14+0.js]{388.45125pt}{270.00875pt}{\ASYprefix cad-14+0.prc}}


==> cad-15+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix cad-15+0_0.pdf}%
}%


==> cad-15.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 80.291010pt{}%
\kern 391.453500pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{12.000000}{14.400000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-195.726750,40.145505)(-0.500000,-0.500000){\includemovie[3Dlights=Headlamp,text={\includegraphics[hiresbb]{"\ASYprefix cad-15+0_0".pdf}},label=,toolbar=false,3Daac=7.360010806366920733,3Dc2c=0 0 1,3Dcoo=0 0 -584.54608996299282353,3Droll=0,3Droo=584.54608996299282353,3Dbg=1 1 1,3Djscript=\ASYprefix cad-15+0.js]{388.45125pt}{77.28875pt}{\ASYprefix cad-15+0.prc}}


==> cad-16+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix cad-16+0_0.pdf}%
}%


==> cad-16.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 74.268500pt{}%
\kern 391.453500pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{12.000000}{14.400000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-195.726750,37.134250)(-0.500000,-0.500000){\includemovie[3Dlights=Headlamp,text={\includegraphics[hiresbb]{"\ASYprefix cad-16+0_0".pdf}},label=,toolbar=false,3Daac=6.86316808445552784,3Dc2c=0 0 1,3Dcoo=0 0 -577.23005456860198592,3Droll=0,3Droo=577.23005456860198592,3Dbg=1 1 1,3Djscript=\ASYprefix cad-16+0.js]{388.45125pt}{71.26625pt}{\ASYprefix cad-16+0.prc}}


==> cad-17+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix cad-17+0_0.pdf}%
}%


==> cad-17.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 150.553500pt{}%
\kern 192.711010pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{12.000000}{14.400000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-96.355505,75.276750)(-0.500000,-0.500000){\includemovie[3Dlights=Headlamp,text={\includegraphics[hiresbb]{"\ASYprefix cad-17+0_0".pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -624.281648950932094522,3Droll=0,3Droo=624.281648950932094522,3Dbg=1 1 1,3Djscript=\ASYprefix cad-17+0.js]{189.70875pt}{147.55125pt}{\ASYprefix cad-17+0.prc}}


==> cad-18+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix cad-18+0_0.pdf}%
}%


==> cad-18.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 156.576000pt{}%
\kern 192.711010pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{12.000000}{14.400000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-96.355505,78.288000)(-0.500000,-0.500000){\includemovie[3Dlights=Headlamp,text={\includegraphics[hiresbb]{"\ASYprefix cad-18+0_0".pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -432.537539634775555442,3Droll=0,3Droo=432.537539634775555442,3Dbg=1 1 1,3Djscript=\ASYprefix cad-18+0.js]{189.70875pt}{153.57375pt}{\ASYprefix cad-18+0.prc}}


==> cad-4+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix cad-4+0_0.pdf}%
}%


==> cad-4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 114.418490pt{}%
\kern 196.726000pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{12.000000}{14.400000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-98.363000,57.209245)(-0.500000,-0.500000){\includemovie[3Dlights=Headlamp,text={\includegraphics[hiresbb]{"\ASYprefix cad-4+0_0".pdf}},label=,toolbar=false,3Daac=28.860495872726254163,3Dc2c=0 0 1,3Dcoo=0 0 -219.37700176381969186,3Droll=0,3Droo=219.37700176381969186,3Dbg=1 1 1,3Djscript=\ASYprefix cad-4+0.js]{193.72375pt}{111.41625pt}{\ASYprefix cad-4+0.prc}}


==> cad-5+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix cad-5+0_0.pdf}%
}%


==> cad-5.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 119.437250pt{}%
\kern 196.726000pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{12.000000}{14.400000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-98.363000,59.718625)(-0.500000,-0.500000){\includemovie[3Dlights=Headlamp,text={\includegraphics[hiresbb]{"\ASYprefix cad-5+0_0".pdf}},label=,toolbar=false,3Daac=5.14449021168138998,3Dc2c=0 0 1,3Dcoo=-24.990342971746400735 11.044142923852394489 -211.841409586314540547,3Droll=0,3Droo=211.841409586314540547,3Dbg=1 1 1,3Djscript=\ASYprefix cad-5+0.js]{193.72375pt}{116.435pt}{\ASYprefix cad-5+0.prc}}


==> cad-6+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix cad-6+0_0.pdf}%
}%


==> cad-6.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix cad-6_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{12.000000}{14.400000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-228.348625,112.415500)(-0.500000,-0.500000){\includemovie[3Dlights=Headlamp,text={},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -500.291931736188473678,3Droll=0,3Droo=500.291931736188473678,3Dbg=1 1 1,3Djscript=\ASYprefix cad-6+0.js]{453.695pt}{221.82875pt}{\ASYprefix cad-6+0.prc}}


==> cad-7+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix cad-7+0_0.pdf}%
}%


==> cad-7.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 156.576000pt{}%
\kern 126.463490pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{12.000000}{14.400000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-63.231745,78.288000)(-0.500000,-0.500000){\includemovie[3Dlights=Headlamp,text={\includegraphics[hiresbb]{"\ASYprefix cad-7+0_0".pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -292.138534403837127229,3Droll=0,3Droo=292.138534403837127229,3Dbg=1 1 1,3Djscript=\ASYprefix cad-7+0.js]{123.46125pt}{153.57375pt}{\ASYprefix cad-7+0.prc}}


==> cad-8+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix cad-8+0_0.pdf}%
}%


==> cad-8.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 155.572250pt{}%
\kern 126.463490pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{12.000000}{14.400000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-63.231745,77.786125)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{"\ASYprefix cad-8+0_0".pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -290.677775485465133443,3Droll=0,3Droo=290.677775485465133443,3Dbg=1 1 1,3Djscript=\ASYprefix cad-8+0.js]{123.46125pt}{152.57pt}{\ASYprefix cad-8+0.prc}}


==> cad-9+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix cad-9+0_0.pdf}%
}%


==> cad-9.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 155.572250pt{}%
\kern 126.463490pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{12.000000}{14.400000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-63.231745,77.786125)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{"\ASYprefix cad-9+0_0".pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -290.677775485465133443,3Droll=0,3Droo=290.677775485465133443,3Dbg=1 1 1,3Djscript=\ASYprefix cad-9+0.js]{123.46125pt}{152.57pt}{\ASYprefix cad-9+0.prc}}

